Operationalizing Research Software for Supply Chain Security

Empirical studies of research software are hard to compare because the literature operationalizes ``research software'' inconsistently. Motivated by the research software supply chain (RSSC) and its security risks, we introduce an RSSC-oriented taxonomy that makes scope and operational boundaries explicit for empirical research software security studies. We conduct a targeted scoping review of recent repository mining and dataset construction studies, extracting each work's definition, inclusion criteria, unit of analysis, and identification heuristics. We synthesize these into a harmonized taxonomy and a mapping that translates prior approaches into shared taxonomy dimensions. We operationalize the taxonomy on a large community-curated corpus from the Research Software Encyclopedia (RSE), producing an annotated dataset, a labeling codebook, and a reproducible labeling pipeline. Finally, we apply OpenSSF Scorecard as a preliminary security analysis to show how repository-centric security signals differ across taxonomy-defined clusters and why taxonomy-aware stratification is necessary for interpreting RSSC security measurements.

==> taxonomy_table.tex <==
\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}
\caption{
Taxonomy categories used to summarize how empirical studies operationalize research software for RSSC analysis.
For each category, we provide a brief definition and representative papers from our scoping set.
}
\label{tab:taxonomy-categories}
\begin{tabular}{p{0.14\linewidth}p{0.16\linewidth}p{0.50\linewidth}p{0.16\linewidth}}
\hline
Dimension & Category & Definition & Papers (count) \\
Supply chain role & build and release & Tooling or infrastructure used to build, test, package, containerize, sign, or publish software artifacts (e.g., CI/CD, build pipelines). & Tam et al; A Curated Dataset of Security Defects in Scientific...; +14 more (17) \\
 & dependency artifact & Software primarily consumed as a dependency by other software (libraries, packages, frameworks). & zhao et al; Harvey, Evan et al.; +1 more (3) \\
 & distribution and governance & Infrastructure or processes for distributing, curating, cataloging, or governing software ecosystems (registries, catalogs, foundations). & kumar et al; Brown, Eva Maxfield et al.; +3 more (5) \\
 & unknown & Insufficient information in the paper snippet to assign a role. & Tsigkanos, Christos et al.; Horvath, Laszlo; +2 more (4) \\
\hline
Distribution pathway & containers & Distributed primarily as container images (e.g., Docker) for deployment or reproducibility. & Tam et al (1) \\
 & installer/binary & Distributed as downloadable binaries or installers. & Urlea et al; Peres, Henrique Estanislau Maldonado et al. (2) \\
 & network service & Delivered as a hosted service or API rather than a packaged artifact. & Green et al; von Kurnatowski, Lynn et al.; +2 more (4) \\
 & package registry (CRAN) & Distributed via a language package registry (CRAN). & kumar et al; Codabux, Zadia et al. (2) \\
 & releases & Distributed via tagged releases and published release artifacts. & A Curated Dataset of Security Defects in Scientific...; Brown et al (2) \\
 & source repo & Distributed primarily via a source code repository (cloned or downloaded). & Sun et al; zhao et al; +4 more (6) \\
 & unknown & Insufficient information in the paper snippet to determine distribution. & smith et al; Peng et al; +9 more (12) \\
\hline
Unit of analysis & award/project & Funded project or award is the analysis unit (e.g., grant-linked software sets). & Brown et al; Harvey, Evan et al. (2) \\
 & code comment & Code comment is the primary analysis unit (e.g., technical debt comment mining). & kumar et al; Codabux, Zadia et al. (2) \\
 & commit & Commit is the primary analysis unit (e.g., change-level mining). & A Curated Dataset of Security Defects in Scientific...; zhao et al; +3 more (5) \\
 & package & Package or library is the primary analysis unit (registry packages, modules). & Sun et al; Green et al; +4 more (6) \\
 & paper-level & Paper or study is the analysis unit (e.g., literature-level synthesis). & Tran et al; Leroy et al; +3 more (5) \\
 & repository & Repository is the primary analysis unit (project-level mining). & Lin et al (1) \\
 & unknown & Insufficient information in the paper snippet to determine the unit of analysis. & Tam et al; smith et al; +5 more (8) \\
\hline
\end{tabular}
\end{table*}

==> taxonomy_table_v3.tex <==
\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}
\caption{
Taxonomy categories used to summarize how empirical studies operationalize research software for RSSC analysis.
For each category, we provide a brief definition and representative papers from our scoping set.
}
\label{tab:taxonomy-categories}
\begin{tabular}{p{0.14\linewidth}p{0.16\linewidth}p{0.50\linewidth}p{0.16\linewidth}}
\hline
Dimension & Category & Definition & Papers (count) \\
\hline
Supply chain role & build and release & Tooling or infrastructure used to build, test, package, containerize, sign, or publish software artifacts (e.g., CI/CD, build pipelines). & \cite{Tam_Chua_Gallagher_Omene_Okun_DiFranzo_Chen_2023a}; \cite{Murphy_Brady_Shamim_Rahman_2020}; +14 more (17) \\
 & dependency artifact & Software primarily consumed as a dependency by other software (libraries, packages, frameworks). & \cite{Zhao_Fard_2025}; \cite{Harvey_Milewicz_Trott_Berger-Vergiat_Rajamanickam_2022}; +1 more (3) \\
 & distribution and governance & Infrastructure or processes for distributing, curating, cataloging, or governing software ecosystems (registries, catalogs, foundations). & \cite{Kumar_Ie_Vidoni_2022}; \cite{Brown_Schwartz_Huang_Weber_2024}; +3 more (5) \\
 & unknown & Insufficient information in the paper snippet to assign a role. & \cite{Tsigkanos_Rani_Muller_Kehrer_2023}; \cite{Horváth_2020}; +2 more (4) \\
\hline
Distribution pathway & containers & Distributed primarily as container images (e.g., Docker) for deployment or reproducibility. & \cite{Tam_Chua_Gallagher_Omene_Okun_DiFranzo_Chen_2023a} (1) \\
 & installer/binary & Distributed as downloadable binaries or installers. & \cite{Urlea_Urlea_Vanderbauwhede_Voinea_Nabi_2025}; \cite{Peres_Galeazzo_daSilvaDantas_Lisboa_deSouzaJunior_2025} (2) \\
 & network service & Delivered as a hosted service or API rather than a packaged artifact. & \cite{Green_Alam_McIntosh-Smith_Gilham_Wishart_2025a}; \cite{vonKurnatowski_Stoffers_Weigel_Meinel_Wasser_Rack_Fiedler_2020}; +2 more (4) \\
 & package registry  & Distributed via a language package registry. & \cite{Kumar_Ie_Vidoni_2022}; \cite{Codabux_Vidoni_Fard_2021} (2) \\
 & releases & Distributed via tagged releases and published release artifacts. & \cite{Murphy_Brady_Shamim_Rahman_2020}; \cite{Brown_Schwartz_Huang_Weber_2024} (2) \\
 & source repo & Distributed primarily via a source code repository (cloned or downloaded). & \cite{Sun_Patil_Li_Guo_Zhou_2025}; \cite{Zhao_Fard_2025}; +4 more (6) \\
 & unknown & Insufficient information in the paper snippet to determine distribution. & \cite{Smith_Zhang_Zhang_McInnes_Keceli_Vasan_Balay_Isaac_Chen_Vishwanath_2025}; \cite{Peng_Kanewala_Niu_2021}; +9 more (12) \\
\hline
Unit of analysis & award/project & Funded project or award is the analysis unit (e.g., grant-linked software sets). & \cite{Brown_Schwartz_Huang_Weber_2024}; \cite{Harvey_Milewicz_Trott_Berger-Vergiat_Rajamanickam_2022} (2) \\
 & code comment & Code comment is the primary analysis unit (e.g., technical debt comment mining). & \cite{Kumar_Ie_Vidoni_2022}; \cite{Codabux_Vidoni_Fard_2021} (2) \\
 & commit & Commit is the primary analysis unit (e.g., change-level mining). & \cite{Murphy_Brady_Shamim_Rahman_2020}; \cite{Zhao_Fard_2025}; +3 more (5) \\
 & package & Package or library is the primary analysis unit (registry packages, modules). & \cite{Sun_Patil_Li_Guo_Zhou_2025}; \cite{Green_Alam_McIntosh-Smith_Gilham_Wishart_2025a}; +4 more (6) \\
 & paper-level & Paper or study is the analysis unit (e.g., literature-level synthesis). & \cite{Tran_Bacher_Shi_Skripchuk_Price_2024}; \cite{Leroy_Combemale_Lelandais_Oudot_2023}; +3 more (5) \\
 & repository & Repository is the primary analysis unit (project-level mining). & \cite{Lin_Peng_Niu_Wang_Liu_2021} (1) \\
 & unknown & Insufficient information in the paper snippet to determine the unit of analysis. & \cite{Tam_Chua_Gallagher_Omene_Okun_DiFranzo_Chen_2023a}; \cite{Smith_Zhang_Zhang_McInnes_Keceli_Vasan_Balay_Isaac_Chen_Vishwanath_2025}; +5 more (8) \\
\hline
\end{tabular}
\end{table*}
